GAN Ensemble for Anomaly Detection

When formulated as an unsupervised learning problem, anomaly detection often requires a model to learn the distribution of normal data. Previous works apply Generative Adversarial Networks (GANs) to anomaly detection tasks and show good performances from these models. Motivated by the observation that GAN ensembles often outperform single GANs in generation tasks, we propose to construct GAN ensembles for anomaly detection. In the proposed method, a group of generators and a group of discriminators are trained together, so every generator gets feedback from multiple discriminators, and vice versa. Compared to a single GAN, a GAN ensemble can better model the distribution of normal data and thus better detect anomalies. Our theoretical analysis of GANs and GAN ensembles explains the role of a GAN discriminator in anomaly detection. In the empirical study, we evaluate ensembles constructed from four types of base models, and the results show that these ensembles clearly outperform single models in a series of tasks of anomaly detection.

==> Figures/mnist-comparison.tex <==
\begin{table*}[t]
\centering
\caption{AUROC results on the MNIST dataset. Ensemble methods generally outperform base models.}
\begin{tabular}{l|cccccccccc|c}
\hline
& 0 & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & average \\\hline
f-AnoGAN & 0.895 &0.699 & 0.863 & 0.785 & 0.781 & \underline{0.761} & 0.896 & 0.702 & \underline{\textbf{0.889}} & 0.630 & 0.799 \\

EGBAD & 0.782 & \underline{0.298} & 0.663 & 0.511 & \underline{0.458} & 0.429 & 0.571 & 0.385 & 0.521 & 0.342 &0.496\\

GANomaly   & 0.881 & \underline{0.661} & \underline{\textbf{0.951}} & 0.796 & 0.809 & 0.868 & 0.859 & 0.671 & 0.653 & 0.533 & 0.673\\\hline
$\text{f-AnoGAN}^\textbf{en}$ & \underline{\textbf{0.961}} & \underline{\textbf{0.943}} & \underline{0.914} & \underline{\textbf{0.913}} & \underline{0.817} & 0.767 & \underline{\textbf{0.957}} & \underline{0.782} & 0.830 & \underline{0.681} & \underline{\textbf{0.857}}\\

$\text{EGBAD}^\textbf{en}$ &  \underline{0.804}&  0.202& \underline{0.671} & \underline{0.577} & 0.438  &\underline{0.480}  &\underline{0.595}  & \underline{0.425} & \underline{0.595}  &\underline{0.458} & \underline{0.525}\\

$\text{GANomaly}^\textbf{en}$   & \underline{0.901} & 0.598 & 0.931 & \underline{0.883} & \underline{\textbf{0.838}} & \underline{\textbf{0.875}} & \underline{0.892} & \underline{\textbf{0.801}} & \underline{0.847}& \underline{\textbf{0.733}} & \underline{0.830}\\\hline
\end{tabular}
\label{table:mnist}
\end{table*}

==> sections/related_work.tex <==
\section{Related Work}
\noindent\textbf{Generative Adversarial Networks (GAN).}
Since the proposal of GANs \citep{goodfellow2014generative}, researchers have been improveing and analyzing the model \cite{gui2020review}.
Recent research shows that mutiple generators improve a GAN's performance in fitting the data distribution \citep{wang2016ensembles,tolstikhin2017adagan,hoang2018mgan}, and multiple discriminators  \citep{durugkar2016generative,neyshabur2017stabilizing} make the training mode stable.  \citet{arora2017generalization} analyze the equilibrium of GAN models and show that a mixture of both generators and discriminators guarantees an approximate equilibrium in the GAN's min-max game. They also empirically show the  multiple at the same time. Our model is based on this type of ensemble.  

%\cite{} propose merely using a single GAN but only differ in the number of training iterations. [Ada Gan] gets inspiration from boosting. They combine potentially weak individual GANs  to form a strong mixture model by running a GAN algorithm on a re-weighted sample. Recent work [MGAN] train multiple generators and a single discriminator during the training. One of the generators will be randomly selected as final output similar to the mechanism of a probabilistic mixture model. The [Discrepancy] argues that explicitly optimizing for the mixture weights once the multiple GANs learned can provide additional improvement.

\noindent\textbf{Anomaly Detection with GANs.}
% Anomaly detection has been investigated in many areas with a a wide range of application especially in computer vision identify.  There already exist a few methodologies that build unsupervised models to estimate a distribution of 'normalness' of data and combine Generative Adversarial Networks(\cite{goodfellow}) and an Encoder-Decoder architecture to detect abnormality by giving scores to samples to m easure how they are biased from  the 'normal' data distribution  (\cite{anogan}, \cite{zenati2018efficient}, \cite{skipganomaly}, \cite{ganomaly}). \textbf{The hypothesis behind those papers} is that if the model fails to recover an input from their captured distribution, it will give a high bias score by matching the high level features extracted from both.
To the best of our knowledge, Schlegl et al.~\citep{f-Anogan} first apply GANs to anomaly detection and propose the AnoGAN algorithm. AnoGAN first fit a normal GAN model over normal samples. To compute the encoding of a training or test sample, AnoGAN needs to optimize a latent vector for the sample through the generator. Then the latent vector of a test sample is compared against latent vectors of normal samples to calculate an anomaly score. F-AnoGAN avoids the problem of optimizing an encoding for every instance by training an encoder for the generator -- the encoder can identify the encoding of a sample. Zenati et al.~\citep{EGBAD} propose the EGBAD method, which trains a BiGAN \citep{donahue2016adversarial} as the model. Then EGBAD compute an anomaly score from the trained BiGAN. Akcay et al.~\cite{akcay2018ganomaly} propose the GANomaly method. The method has an encoder-decoder [cite] as the generator and trains a separate encoder for reconstructions. This method compares samples in the embedding space to compute anomaly scores. \citep{akccay2019skip} further improve the GANomaly method by replacing the encoder-decoder with a U-Net \citep{ronneberger2015u}. 

% However,  these models \textbf{cannot capture the real distributions of the normal data}. It is hard to avoid overfitting because the normal training data do not always represent the exact distribution over all normal data. As a result, these models may be too confident on their prediction result and fail to recognize  unseen normal data and output a high abnormal score.

% Bayesian approaches can help the model to give a confidence score for its predictions. Generative Adversarial Network can help the Generator capture the distribution of the dataset by performing a min-max game during training process. Encoder-decoder architecture is good at extracting useful information from high dimensional space and reducing it into a low dimensional space, and has been widely used in many image inpainting and image denosing problems. In the past research, there have been a few works on anomaly detection by combining bayesian approaches, GANs and other encoder-decoder architectures (\cite{bayesiangan}, \cite{ganomaly}, \cite{skipganomaly},  \cite{anogan}).

% We introduce a Bayesian GAN Encoder-Decoder Convolutional (B-GEDC) neural network to estimate the distribution of normal or typical data examples in the training data  as much as possible while avoiding overfitting.

% During the training process, we only use normal samples to train B-GEDC model. During evaluation, when an unseen test data is fed to the model, the model's prediction  is not determined by a single discriminative model but by both a mean abnormal score and variance (i.e. confidence) over all sampled models.

% Our hypothesis is that, by the application of bayesian approaches, B-GEDC model can get a more reliable and solid distribution of normality on the training data, regardless of the size of the training data.

% The proposed method with a better result doesn't rely on innovation of neural network structure, but on \textbf{change of training process}. Our model's uncertainties in estimated probabilities are better. 
%\paragraph{Ensembles of Generative Adversarial Networks}
% By using an ensemble of GANs, it has been proved by multiple researches having the potential to resolve the problem of missing modes that frequently occurs when training a single GAN. Mode collapse has a significantly negative influence for abnormal detection task since it will miss some normal distribution and cause misunderstanding during the inference stage. [https://arxiv.org/pdf/1612.00991.pdf] propose simply using a single GAN but  only differ in the number
% of training iterations. [Ada Gan] gets inspiration from boosting. They combine potentially weak
% individual GANs  to form a strong  mixture model by running a GAN algorithm on a re-weighted
% sample. Recent work [MGAN] train multiple generators and a single discriminator during the training. One of the generator will be randomly selected as final output similar to the mechanism of a probabilistic mixture model. The [Discrepancy] argues that explicitly optimizing for the mixture weights once the multiple GANs  learned can provide additional improvement.




